Human-Computer Insurrection: Notes on an Anarchist HCI

The HCI community has worked to expand and improve our consideration of the societal implications of our work and our corresponding responsibilities. Despite this increased engagement, HCI continues to lack an explicitly articulated politic, which we argue re-inscribes and amplifies systemic oppression. In this paper, we set out an explicit political vision of an HCI grounded in emancipatory autonomy - an anarchist HCI, aimed at dismantling all oppressive systems by mandating suspicion of and a reckoning with imbalanced distributions of power. We outline some of the principles and accountability mechanisms that constitute an anarchist HCI. We offer a potential framework for radically reorienting the field towards creating prefigurative counterpower - systems and spaces that exemplify the world we wish to see, as we go about building the revolution in increment.

==> sections/scraps.tex <==
\section{Scraps}

...It has also seen a resurgence within academia (never immune to anarchist philosophy, with the field of geography originating in the work of Kropotkin, a prominent anarchist thinker \cite{Springer2012}) – geographers, sociologists and anthropologists have all recently pushed for anarchist approaches to their field (Ince, 2010; Purkis, "towards an anarchist sociology", in Purkis \& Bowen, 2013; Graeber, 2004).
% \section{Anarchist Metrics for Evaluating HCI Work}
% \textcolor{blue}{Do these still fit at all?  If so, where do they fit into the new structure of world -> community -> self?}
% % \subsection{Sustained Critical Inquiry}

% %\footnote{'hermeneutics of suspicion' == critique of postcolonialism}
% Drawing on the ideas of embodiment and contingency, critical theories such as the feminist philosophy of a successor science could represent one spoke of an evaluation metric for anarchist HCI. Harrison et al. cite Harding??'s description of feminist successor science, defining it as the creation of new forms of science that work in opposition to codified scientific mechanisms and norms relying on gender, class, racial, and other biases. Rather than striving for objectivity or universal truths, successor science principles dictate that biases and contexts should be explicitly acknowledged [Harrison et al., 2011]. Moreover, these approaches necessitate ongoing reflection and critical engagement to ensure appropriate rigor. According to Haraway, the foundations for credible claims of objectivity include both hope for transformative knowledge and sustained critical inquiry~\cite{haraway1988situated}. These disciplines are particularly concerned with exploring and representing the perspectives of groups whose ideas and experiences have been marginalized in mainstream or canonized discourse. Yet, as Haraway argues, the fact that an account is drawn from an underrepresented community does not in and of itself make it credible. She cites Marxism as one approach toward critical interrogation of these situated knowledges, and thus a good starting point for the "feminist version of objectivity:" Marxism, she asserts, offers "a rich tradition of critiquing hegemony without disempowering positivisms and relativists and a way to get to nuanced theories of mediation" [Haraway, 1988].
                    
% The principles of successor science seem to fit well with new HCI theories including participatory design, postcolonial computing, and critical design. The overarching goal of most of these new approaches is to design well for a particular context, rather than designing for (or even assuming there is a universally appropriate design methodology. Harrison et al. claim that these principles can be viewed as elements of a unified framework that "treats interaction as a form of embodied meaning-making in which the artifact, its context, and its study are mutually defining and subject to multiple interpretations" [Harrison et al., 2011]. This view of agency is closely aligned with Suchman's, yet combined with the mandate for critical inquiry, it opens up more avenues for self-determination and widespread participation in the making, reshaping, and rejection of <HCI interventions>.   

% ((It should be noted that the Harrison et al. paper is a far cry from anarchist HCI. But it does start to synthesize ideas from Bardzell's Feminist HCI, Irani's postcolonial computing, standpoint epistemology, etc.  May fit better in the earlier section around values-centered HCI, but I think we should reference again as part of our metrics for evaluating anarchist HCI))

% Should include the trio of options from the anarchism and technology paper about responses to tech (Gordon, 2009)
% \subsection{Recognition of Funders and Relationship to Capitalism and the State}
% Affirmative demonstration that results/methods/tools/etc. are not driven by funder demands or perceived expectations.  Demonstration of ways that work challenges or at a minimum does not serve capitalist or state interests.

% the right of reply \cite{Fox2016}

% Methods
% Demonstrate how concerned parties have participated in the work and are directly served by it.  Include commentary from participants and insure they are compensated for this work.
% What else?    


%\footnote{and HERE is where we subsection and launch into discussions of work shifts, design shifts and changes in accountability and expectations, which nicely segues into discussing accountability mechanisms!}
\subsection{anarchist communities scraps}
"We can ask how local groups actually are conceptualizing a shared idea of a public interest, right now, in the absence of State mediation. We can do this because even though we live in a society governed by a State, the State is not ubiq- uitous. In principle, every relation in its territory is subject to its sovereignty, but of course, in practice, the State is not always there, not always judging, deciding, and gov- erning. There are countless examples of people working out questions like this for them- selves, without any significant involvement by the State. These examples range from the mundane (neighbors negotiating how to use the parking spaces on their street) to the spectacular (people in informal settlements figuring out how to hook up and regulate an electrical system for tens of thousands of people). These kind of relations, both among communities and between smaller communities and wider publics, are being negotiated all the time, in real life, without the State, by urban inhabitants themselves. And so the empirical habit of thought here is: pay attention to these practices. We do not have to assume that life without the State only exists in the unrealistic fantasies of anarchists. Life without the State is, instead, a very real and very common fact of life. Publics with- out the State are being created and negotiated all the time, and in our empirical research we can choose to pay attention to them, record them, narrative them, compare them, and learn from them." \cite{Purcell2016}

\subsection{Theory of an anarchist HCI scraps}


marginalization would be foregrounded, no longer sufficient for 3d printing to make argument that it's emancipatory because it redistributes production of stuff without interrogating embodying/confronting for whom

confronting marginalization as a requirement for any work, rather than a point of critique for existing work.  

infrastructural and technical sophistication predicated on colonialism and exploitation? if we want HCI to genuinely be accessible to everyone, we have to confront ecological and resource limitations.  some things aren't possible in the current strictures.

cue for discussions of some things aren't possible because infrastructure inherently concentrates and fixes power, require new ways of organizing the world

decentralization of tools as well as products and the associated risks

*messianic designer narrative*
designer as manager of priorities (VSD - Meg will check notes)

professional working relationships, what does it mean that our conferences so heavily concentrated that are dedicated conferences elsewhere ((not sure this is actually illustrative of the problem))

grant money, association with industry

``the anarchist squint" james scott

gender in HCI - range of epistemic traditions - we implicitly understand our norms and values to be universal even when we explicitly state otherwise

gender hci, normative definitions and the power to define knowledges, epistemic power, norms and meanings assumed to be universal, canonical

power includes the power to define knowledge

Things do not need to change that much - theorists note many of the 'alternative' forms of organisation we already engage in as a society are anarchistic in nature, or could be~\cite{White2014, White2012}.


What might a theory of anarchist HCI look like?~

%\footnote{JH:  anarchism aligns nicely with newer design theories (design justice, post-capitalist, etc)
%- anarchism cares about power so inherently could be used as a grounding for feminist/trans/race/disability HCI
%- Calls for us to revisit how power appears in our own field
%- grounding of an anarchist HCI is how a piece of work reduces power inequities and builds counterpower
%- technochauvinism concerns}~\footnote{JH: development of "low theory" [c \& g article/graeber]} (Well, let’s also see what we pull out for values and grounding from the "what is anarchism?" section \& get more precise with the anarchism part).        
"What does it do to our research to attach it to varied political agendas rather than burying the lead under seemingly objective values of efficiency or utility? [Irani, commentary on AnarCHI]"
A theory of anarchist HCI would articulate what "there" we might be getting to; with what do we replace capitalism? ("That’s how we’re gonna win. Not fighting what we hate, saving what we love" OKAY AND ALSO FIGHTING WHAT WE HATE). For what new world are we challenging "larger structures" (DO WE WANT TO LIVE IN THE CULTURE OR ANARRES AND WE ARE NOT PROPOSING A FEUDALIST HCI)? How do we communicate these to each other? How do we resist the formation of new "larger structures (postcap)" in examination and in action (e.g. active revolution)? How do we ensure that we're not just confronting an economic theory, but a political one? What philosophy best guides our relationships, activities, and creations? How do we evaluate our work and world?
Theory for revolutionary action, theory for world-building ("utopia as cognition")
Bardzell: What a world might look like— Utopias paper talks about the importance of "Utopia as Cognitive Act" to help
Post-Capitalist HCI cites the iterations \& "grand visions" paper 
Feenberg’s critical theory of technology lays some groundwork for this, but stops short of challenging the structure of the state.  "The means of democratic expression on technical issues are already foreshadowed in many current practices such as hearings, citizen juries, technical controversies, protests, boycotts and legal challenges, hacking and other creative appropriations of technologies, and of course such familiar methods as elections and government regulation" (Feenberg 2010).
An anarchist HCI must compel an unflinching interrogation of power and an unceasing motion toward liberation—"forever looping contestation [Adversarial Design]" ("movement never lies")
"Attempts to create autonomous communities in the face of power (using Castoriadis’ definition here: ones that constitute themselves, collectively make their own rules or principles of operation, and continually reexamine them), would, for instance, be almost by definition revolutionary acts. And history shows us that the continual accumulation of such acts can change (almost) everything. [DG, F]" ("You can pull the trigger or you can build you an ark", JM—DESIGN IS LIBERATORY IF IT SAVES PEOPLE)
Several theoretical branches within HCI are critical of inequalities and oppression, sometimes directly identifying capitalism and the state as actors and infrastructure of our oppression—an anarchist HCI is compatible with the agendas of Feminist/trans/race/disability/post/anti-colonial HCI, Design Justice movement, "Humanity-Centered Design", "Design for Social Justice", "Equity Design" 
A theory of anarchist HCI would provide a sharper focus to this critique, offering a precise definition of oppression and attention to ways it might manifest
A theory of HCI would offer an explicit definition of liberation, rooted in autonomy and communalism (a condition of which is the destruction of capital and the state) \footnote{OK: Would also, by centering power as a measure of outcome, avoid the difficult neoliberali idea of liberation consisting of assimilation into structures that perpetuate harm (mandatory cite to 'knocking the hustle') JH: Yes! I totally didn't get to outcome and evaluation, but I think that's important to offer (and a nice dialogue with the conclusion of last Design Justice paper)}
"The process of decolonizing design makes it into a space where every future may exist, insofar as every future has its de/ futuring character challenged. Moreover, the exhibition/observer format frequently found in design discourses must be questioned, and borders among the visitor, the object, and the author[ity] torn down. The designer must cease to be the sole narrator of a story. The act of designing objects, services, scenarios, and speculations for the future must be reframed to facilitate debate and action" [O Martins and Oliveira, 2016].
                        
Anarchist HCI cannot be decoupled as a theory and a practice; anarchism demands urgency and commitment to challenging domination.

\subsection{Anarchist HCI in Practice}
Practice of an anarchist HCI %\footnote{JH: -ideas for ways it'd impact subfields
-ideas for projects we could undertake
-techniques/changes to the field itself (accountability, practices between academics, funding)}

We want to talk about PREFIGURATION, the reflection of a movement’s desired future in internal practice/’creating unknown futures in the present’ (Ince, 2010)
What might a practice of anarchist HCI look like?
Anarchism doesn’t look like one thing! 
We’re advocating for specificity of political philosophy, towards a clarity of desired conditions and values, not a particular arrangement. "Utopia as Cognitive Act"
An anarchist HCI would commit to the abolition of capital and the state and all hierarchical power structures %\footnote{OK: Do we wanna explicitly reference the danger of ignoring implicit rather than formalised power structures, and shape our language to include both? JH: Yes! I think that will be key to not being dismissed, and also not being, I also think that implicit power connects to things like our research and design motivations (moving from "nothing about us without us" to "by us for us" or something? with active, ongoing, enthusiastic consent) and to things like, persuasive design (I like hacking my own brain, but I have my full consent insofar as I am not influenced by social pressures, blah blah and like, tactics can be valuable but we should at least understand the cost).}
\& a core philosophy based on values of free association, cooperation 
Might look like: "Small projects, Big ideas and a vow
Use our tools to provoke and protest
And use computers to make futures that are ours" [anarCHI]
"We encourage research motivated by passion and dissent over patents."    
 "... one must oneself, in relations with one's friends and allies, embody the society one wishes to create." ― David Graeber, Fragments of an Anarchist Anthropology
Disruption of our own hierarchy
Shift from colleague to collaborator ("collaborator" subtext meh, please don’t make me say "comrade")
Move from "design with not for [McCann]" to something more direct, less interventionist at all?
Confronts solutionism and techno-chauvinism - this is both systemic and endemic as weird gross culture maybe because we try to position ourselves as counter to capital but uh, we are not (heyyy hackathon paper, heyyy counterculture computer, heyyy whatever origins can be another paper)
Direct acknowledgement and ongoing interrogation of power within and across all sociotechnical systems
Rethinking what technology is, does, and who it’s for
Transparency and honesty―we need a reckoning if we’re going to do this work
We have to focus on the most marginalized―because survival, and because this is how we continually interrogate the roots of power structures/prevent emergence
Refusing to participate/funding ("Tech Won’t Build It")
When the implication is not to design
When the blah blah is to destroy (setting up counterpower as a method--willingness to trash our own work?) \footnote{Undesigning technology: considering the negation of design by design}
An anarchist HCI would require new or radically altered design methods—current approaches were developed within and for current world, with all the attendant power relations (including reduction to transaction between designer/user)
What might anarchist design methods look like? What might they seek to do? \footnote{OK: I wonder if Sasha has anything on this given their use of zapatismo}
"revolutionary action is any collective action which rejects, and therefore confronts, some form of power or domination and in doing so, reconstitutes social relations—even within the collectivity—in that light [DG]"
Prefigurative %\footnote{JH: "Likewise, we can begin to imagine a corollary to prefigurative politics through a notional prefigurative design, where design work that is explicitly oriented in service of political or civic goals does not only articulate or represent these goals as design objects, and instead structures design processes to do the work of trying to actualize them. This stands in contrast to human-centered design practices which position themselves outside the frame of use—experience, use, and values are extracted through an attenuated design process as raw material to inform the design. Prefigurative design, on the other hand, exists within the design frame and enacts the experiences, uses, and values in the design process rather than only in the articulation of the system or artifact.
%The design work we have presented here follows the traditions of participatory design with some affinity toward speculative design. From the former, it borrows the mechanisms of stakeholder participation and collaboration to build outcomes that both reflect and benefit those involved in the process. From the latter, it borrows the vision, creativity, and radicalism of imagining and creating an alternative future. Returning to the anarchist roots of prefigurative politics, prefigurative design both anticipates an alternative future and changes current circumstances to better resemble this anticipated future [9,14]." - SOCIOTECHNICAL API PAPER}
%Insurrectionary Anarchism? dismantling/critical/speculative
%(I feel like there is something to Graeber’s statement about how a lot has been accomplished by posing alternatives/opting-out (oh, hey double parenthetical also Doctorow’s flawed-but-endearing novel "Walkaway"—we can directly attack, and we can also build something else—this is about both immediate survival and imagination per theory) \footnote{OK: The technical term we want here that we probably want to bring out a lot is 'counterpower' - the construction of alternatives to inherently reduce the power of the state in any situation where choice is even theoretically available. JH: I also want to explore counterpower as manifest (like, interventions/insurrections, etc.) and as what we construct in our imaginations (e.g. what can we envision...re: Bardzell's call, sentiment like "it matters what blank blanks blank", and also just general interest in representation, narrative, etc. but that may be too far afield). OK: so tbh I'd argue insurrections aren't inherently counterpower, they're the thing you enable through counterpower? that might be wrong but. JH: I think that's a good point...and I think I'm thinking broadly (but not sure how to articulate) about a variety of actions (that may not be counterpower): build alternatives (maybe this is more explicit counterpower?), challenge existing power in ways that rebalance and erode structures long term, block something immediately harmful by those in power/reduce power in a moment or remind those with power that they are vulnerable (which are balancing in a way but may not see an immediate measurable outcome in the system or may even see backlash), actions that "prefigure" (YAAAY words) and create the conditions for us to do all this work, and actions that help us envision/think about/imagine a world with all of these things...and these aren't all mutually exclusive. But I have to do some reading because I'm sure this has been addressed in many contexts from anarchism to just...design methodology.}
In an anarchist HCI, participatory design becomes...what? %\footnote{OK: we might wanna include stuff on researcher care and ethics here too. JH: Oh gosh, yes. I hadn't even thought about how breaking down divisions mandates self-care, too, because we aren't taking on a mantle of "vocational devotion" because without "professionalization" something about "self-interest vs community interest" collapses.} Or...there is no co-design, only design? (Critiquing professionalized "design" as profession: Irani, Bardzells (RTD?), Costanza-Chock, Rosner, hackathon paper...connected to what expertise is valued, lived experience as knowledge, move from "design with not for" to "stop implying hierarchy just because specialization") \footnote{JH: NTS, this may be another jumping off point: "In reconfiguring this terrain to explicitly recenter the margins, feminist hackathons are able to invite modes of thinking previously devalued by positivist models, including non-technical approaches and partnerships between citizens and established community activists [3, 6, 12, 13] as subject-matter experts and co-designers. With this remaking, designers and technologists are no longer gatekeepers of knowledge or production, but potential (rather than necessary) collaborators. And they, too, may find that their vocational knowledge and output is valued as secondary to the contributions and perspectives they can offer as individuals or members of communities."}
"the only plausible solution: collaboration between the concerned groups and professional specialists" [Callon, 2010]
Fox \& Le Dantec - Community Historians paper
How do we reconcile this stance with our own positions wrt to design and research? %\footnote{JH: This is so vital. Also I think we can pull this in re: some of the punk HCI feedback that I found interesting (and maybe we address this in multiple places, as limitations, an example of doing this work even without having answers because we are seeking the journey and as contextualizing/reframing anarchism):

%"Along these lines, though, we are forced to question whether this paper should really be seen as anarchist. It strikes us as highly unlikely that anarchists would write an abstract or present anything in the SIGCHI Extended Abstracts format. Anarchists might be more likely to show up at the conference and run their own session, maybe in the lobby or even outside the convention center, where they bring their own soapbox to stand up and say what they want to say. Or, perhaps more in the vein of corporate sabotage, anarchists might switch the labels on different rooms or introduce errors into the printed program so that people wanting to attend one session actually end up in a different room." MD: [Running their own parallel session] is sort of a thing that is happening....not from an anarchist framework, but actually I think Sarah Fox and Amanda Menking (:/) were talking about doing this last year...not sure how it panned out because I think it was supposed to be at CSCW and I didn't go this past year.}  How do we avoid implying hierarchy if we are speaking to an academic audience?  Where does this discussion belong?  Is it in a limitations section or up front as part of our outlining the problem?
%Making reimagined as truly liberatory? Or challenge of property? \footnote{MD: Values in Repair paper? Also what markers are we using to distinguish maker movement from a liberatory practice of making? Barriers to access? Hierarchies in status of different types of making? JH: Yes to Values in Repair paper! I'd say the critiques of making at large germane to this definitely include barriers to access and hierarchies in status (e.g. "Make" vs "Craft") but also much of the Maker movement's reliance on industry production and its failure to contend with sustainability/responsibility for impacts; colonialism; focus on "American" narrative/mythologizing of the "neolibertarian" ethos.

%Bardzell et al. "HCI's Making Agendas", Ames, Bardzell et al. paper "Making and Making Do..." and "HCI after technosolutionism" can help frame some specific distinguishing potential between the current reality and potential for a liberatory practice of making. MH: There was a Forum on Design as Inquiry that addressed some of this. Also Kathryn Shroyer's work is closely related, but I'm not sure which projects are published yet}
What might happen to some subfields?

Productivity-related IS GONE (Just...gone because work!)
Ubiquitous computing becomes NOPE (we’d be called to interrogate not only the conditions which support a particular vision of ubiquitous computing, but the concept of ubiquity itself—e.g. the desire for automation and convenience—and really, technological interventions—isn’t universal) \footnote{OK: and universal requires ubiquitous control. JH: It does, but does it have to? (I think that's another paper about fully automated luxury blah blah, hahaha). Or rather, does ubiquity have to imply universalism?

But back on topic, yes we would need to develop process, artifacts, systems, etc. while avoiding centralized control and the ability to withdraw consent, etc.}
Gender HCI? I bet we could say some interesting things around how that would be reshaped that would make a lot of people very mad
There’s the Winner thing about technologies and infrastructures not being as possible without hierarchy

\textbf{anarchist squint~\cite{Scott2018} and hermeneutics of suspicion~\cite{bardzell2015humanistic}} 
\textcolor{blue}{
After reading through several sections of Scott's work, I'm not sure how we meant to relate the anarchist squint to the hermeneutics of suspicion.  Perhaps we meant that the anarchist lens was a layer on top of the hermeneutics of suspicion? ((Re-reading the sections of Bardzell work on hermeneutics of suspicion...will synthesize ASAP))
}

\section{The Politics of HCI}

\begin{quotation}
\textit{"You are ultimately-consciously or unconsciously - salesmen for a delusive ballet in the ideas of democracy, equal opportunity and free enterprise among people who haven't the possibility of profiting from these."} \cite{Illich1968}
\end{quotation}

% \subsection{HCI for Social Change/HCI as Situated in Particular Social Contexts}
% The last few decades have seen HCI take a turn to examine the societal implications of our work; who is included\cite{Amagno2012, Hankerson2016, Hayes2015, Irani2016}, what values it promotes or embodies \cite{Shilton2018, Friedman2002, Friedman2017}, and how we respond (or do not) to shifts in outside society (Light, 2017). This work is laudable and necessary, and has to some degree even been given "official" backing (see, for example, the CHI4Good conference[cite])\footnote{Possibly add Rosner 2018; Le Dantec; Dombrowski et al. 2016; Baumer \& Silberman 2011, maybe Houston et al. 2016; Luger \& Rodden 2014; }
 
% \subsection{Acknowledgement, but Failure to Engage with "Constraints" of Existing Structures}
% But this work is also limited, constrained: time after time,\footnote{MD: need to cite other examples to validate this statement} a reader of works on values-driven HCI will run into a statement such as:
 
% Finally, it is important to acknowledge the limits of a values-oriented approach to design...values-oriented approaches do not address larger power structures that perpetuate bias and unfairness in technology hiring practices, design education, or technology regulation\cite{Shilton2018}.
 
% \subsection{Failure to Recognize Implications of Power Structures}
% Alternately there will be no such statement, reflecting not an avoidance of these "larger power structures" but an avoidance of recognising them. The result is papers (for example) look at improving the gender-accessibility of software through a company that received 238 gender discrimination and harassment complaints in 2018 from its own employees \cite{Burnett2017} \footnote{news cites go here}, or the "empathy" of design through legitimising security systems with long-established racist and transphobic biases.\footnote{OS: news cites go here and also that design thinking book MD: add engineering education (Cech). Also, fuck AT. To what extent do we want to get into HCI’s articulations of agency in interactions with technology?  I would argue that several of the most prominent HCI theories belong in this category of failing to recognize larger power structures (e.g., Kaptelinin \& Nardi on AT, Hutchens and others on DCog, Suchman on posthuman agency)} %\footnote {JH: Not that it inherently conflicts because values in pluralism, flux, autonomy, rather than an end goal but speculative design (or at least, Dunne \& Raby) seems committed to the provocation and conversation without necessarily taking a stand on doing the work of articulating a set of values, which feels like it runs into this wall. Explicitly critical designs may face less of this, but that's still the critical rather than the insurrectionary? Not sure where I was going with this. I think Bardzell's PD piece also gives examples of failure to engage with constraints (or scale). MD: There are actually several(not actually sure how many? maybe just a few important ones?) critiques on Dunne \& Raby for exactly this reason.} %\footnote{MDL also maybe the 2004 DIS panel "Beyond Human-Centered Design?" It is ick}

% \subsection{Conciliatory Transition?}
% To a certain degree both responses are understandable (although one certainly more laudable): we should recognise our constraints, and we do sometimes have to undertake work that [some idiom goes here about, like, two steps forward one step back]. But what comes after that? %\footnote{JH: Maybe this is a place to bring in the design futuring iterations vs. grand vision that inspired the post-capitalist HCI workshop? Like, it's kind of the reform vs. revolution but I think instead we're trying to say let's re-scope the definition of a revolutionary act, per Graeber and counter power, freeing our imaginations, reducing daily suffering, etc.?}
% In HCI the answer is often "nothing": our works frequently include the requisite Winner citation \cite{Winner1980}, but beyond that rarely engage with politics in the sense of challenging these "larger power structures", or working to articulate visions of the world we would like to see and the specific actions that can be taken to get there.

% \subsection{Addressing Politics and Values of HCI Explicitly}
% Even on those few occasions where explicitly-political theories (Marxist analysis, for example) %\footnote{MD: Do we have an example of some of these works? PD HCI works bring Marxist analysis in explicitly, don't they?}
% are brought into HCI, they are done so quietly and without naming. But this does not mean that the field lacks a politic: on the contrary, ``any social or cultural analysis that does not engage politics is almost certainly ideological itself''~\cite{Bardzell2015}. Within HCI all suggestions are that this consists of an ``implicit neoliberalism''~\cite{Feltwell2018}, which (in a world of explicit neoliberalism) inherently constrains us to not challenge those "larger structures".%\footnote{MD: Add points on situated knowledge, epistemological trouble (Harrison 2011; Haraway) Is Feminist HCI already in here somewhere? (Bardzell 2010; Suchman; Balsamo 2011)}

% There are signs this is changing. Bardzell \& Bardzell's ``Humanistic HCI'' and its call for an explicitly ``emancipatory'' HCI is the most comprehensive example of this, and advocates a ``hermeneutics of suspicion'' which pushes us to effect substantive change. ``Post-Capitalist HCI''~\cite{Feltwell2018} and the (admittedly, tongue-in-cheek) anarCHI paper~\cite{Linehan2014} offer visions of a world without capitalism, or the state. But none of them go quite far enough: Bardzell \& Bardzell talk broadly about a range of possible analytical methods, without discussing what a world in which those are deployed might look like, while "Post-Capitalist HCI" envisions a world in which these "larger structures" have been challenged but does not (guillotines notwithstanding~\cite{Pettitt2018}) suggest how we might get there.
 
% The goal of this paper %\footnote{JH: Placeholder comment/thoughts that may very well go nowhere:

%1. While some outcomes of the workshop may have posited a post-state vision, the workshop call was broader ("Post-capitalism is the proposal of a socio-economic model that completely replaces capital as the primary method of organising society. This idea is not new - Marx and Engels wrote at length about the destruction, replacement or evolution away from capitalism towards a society where humans are freed of labour by the technological advances of the time. This work, along with social experiments such as the Paris Commune [19] helped to progress and disseminate understanding of alternate socio-economic systems, such as socialism, communism and anarchism. Each of these represents a specific vision of a post-capitalist society, with their own histories of implementation and evaluation.") So this was a necessary move forward and we're saying, yes and the specific vision we want is this because post-capitalism is great but we need to contend with more.

%2. Post-Capitalist HCI workshop saw a need for "grand visions" and not only projections, which is awesome and true, but can specific political philosophy as a framework and grand vision help HCI bring the vision into "projection" that serves as counterpower? (this also connects to Bardzell's "Utopia as cognitive act"-not that we have to use any of that, but just the value of imagination, representation, etc. that help us have the pathways to even think about what's possible--e.g. the Post-Capitalist HCI workshop cites LeGuin. - There is a lot around design fictions and speculative design and narrative and storytelling and representation but that's a lot of threads to pull on. I think I just want to communicate that a political philosophy is a grand vision AND a grounding for our daily work in a very tangible way.} \footnote{MD: I think this belongs in the intro. Also, are we necessarily speaking only to researchers?} is to tie methods and outcomes together by discussing a specific political vision for the field - specifically, in line with the pointers towards an "emancipatory" HCI examining structural power (particularly that of capitalism and the state), a vision of anarchist HCI. This, we hope, can be seen not just as a particular model of "emancipatory HCI", for "emancipatory HCI researchers" to adopt while the rest of the field returns to its usual business, but as a start in researchers across our field beginning to ask themselves what politics their works embody, and ask the same of the research they review. [this is a bit big]
 
%While we do not expect many readers to be familiar with anarchist theory (and many more to be sceptical!) the idea is not as far-fetched as it sounds: political fields have often incorporated anarchist lenses on the world(), and most prominently (in the case of geography) been explicitly founded by anarchists (Springer, 2012). [this might go better in the beginning of the second section] also the anarchist theorists are already thinking about tech, one half of this is already there. \footnote{MD: Could we also point toward some ways to force industry/state actors to grapple with their politics, or is this intended to go later in the paper? Mechanisms that undermine exploitation from industry/state actors (e.g., H1N0) Mechanisms for transparency "Alternative" technologies or ways to participate in technology design that facilitate divestment from [the imperialist, capitalist, ableist, hetero-normative, patriarchal, white-supremacist machine] (Erynn Brook's adaptation of bell hooks descriptor). OK: I sort of had it mentally fitted in the 'us pitching examples of ways practice could change' but if we're focusing instead on in-field changes to what we work on and how, it could fit here. JH: Also Design Justice references Collins' "matrix of domination" (white supremacy, heteropatriarchy, capitalism, and settler colonialism)}


% \subsubsection{Process/Organization}
% \textcolor{blue}{MD: Make sure this is in the anarchist HCI section somewhere}
% Conferences as a mode of knowledge transfer, communication, networking, etc - limits access: we have this weird hierarchy between "real CHI" and "sub CHIs". The main chi is promoted; the others are not. There is an inequivalence of knowledge validity. People can push back and say "well, there are different review standards etc" but it doesn't just look like review standards, it looks like a privileging of the US and EU. It is noticeable that there is no US "sub chi". We don't need one: when the CHI chair's report locks in a minimum of 2 CHIs in north america in the next five years, our sub chi is REAL CHI. The result is a privileging of the same sources of knowledge in validation, publicity access+networking year in year out, as evidenced by the tables of whose papers appear at "main chi". Also sets up a dichotomy for researchers: in the presence of limited funds, do you want to go present at CHI+circulate work or invest in your research. plays into tensions+difficulties with eg use of mechanical turk. Also why are they all in english???? eat my entire ass. ALL OF IT. EVERY LAST SQUARE CENTIMETER OF ASS. TRY PUTTING SOME PASTRAMI ON IT IT'LL GO DOWN EASIER.



% \textcolor{blue}{Transition: What does it mean that HCI has put forward equity/social good/empowerment as ideals of our work? Transitioning to the critiques scholars have raised with myopia, privilege-blindness, ``apolitical'' approaches, etc.}



% \subsection{Our Contributions}
% Marxist Lens is Necessary but Insufficient to Challenge Larger Structures of Oppression\footnote{Does this actually need to be said or is it self-evident?}

% A Coherent Vision for HCI that doesn't make the world worse

% Marxist analytical lens + design justice principles and methods = a coherent narrative for HCI work that isn't reinforcing systems of oppression and that is doing its best to undermine them.  We are working with explicitly political and utopian goals.  We are going on record that justice is fundamentally not possible under capitalism or the state.

% Concretizing Methods of Evaluation and Accountability
% By laying out specific metrics for evaluation that would fall under an anarchist HCI, we can force/compel/encourage\footnote{force, anarchism...eh} researchers and practitioners to either explicitly or implicitly confront the lens through which they view the world and their work in HCI.  

%\footnote{JH: Do we want to talk about insurrectionary anarchism? And/or what do we want to say about it/tensions? Approaching this from theory/practice of directly and continually dissolving power , as adversarial design (``forever looping contestation [AD book]") /critical design as provocation and I’m thinking about Irani’s ``Critical Design to Critical Infrastructure" paper-which is kind of a bridge) 
%be sure to incorporate queer/black/etc anarchism
%What are the threads we want to identify as salient for our own values?
%Vision/Philosophy
%A iff B
%Tactics, centering, common organizational structures, or lack of same
%}

%\textcolor{blue}{
% The broader categories under which third paradigm HCI theories fall, according to both Rogers and Steve Harrison, 
% also deal explicitly with self-reflection as a key component of the design process.  Harrison argues that 
% third paradigm theories that have previously been considered unrelated actually fit within the feminist philosophy 
% of successor 
% science.  Successor science, as Harrison summarizes it, is the creation of new forms of science that work 
% in opposition to codified scientific mechanisms and norms relying on gender, class, racial, and other biases.  
% Rather than striving for objectivity or universal truths, successor science principles dictate that biases and 
% contexts should be explicitly acknowledged~\cite[p. 387-389]{harrison2011making}.  Rogers explains a similar 
% umbrella term for third paradigm HCI: critical theory.  
% }

% During the same period in which HCI turned toward the social, Cech noted how a "culture of disengagement" in engineering education has reduced consciousness around the societal impacts of engineering work. This culture derives from ideologies and rhetoric that draw arbitrary distinctions between the technical and the social, treating technical work as serious, objective, and apolitical, whereas ``social'' work is devalued~\cite{cech2014culture}. Given HCI's closeness to engineering, it is not surprising that the HCI community might similarly struggle to reckon with the social impacts of our work. A variety of theoretical approaches to HCI and design have arisen to bridge the false dichotomy of the technical and social.


\textcolor{blue}{
These researchers (and many others) are responding to the needs of communities within which they belong and work, working from different critical lenses to produce tangible  interventions with positive social aims [???]. But the precise politics manifested by these works are often implicit; with few exceptions (such as Asad's work on community engagement, which specifically points to anarchist principles of "prefigurative politics" and posits a "prefigurative design"~\cite{asad2017creating}), we neglect to explicate our political vision: how it informs our focus, shapes our processes, and how our work should contribute to its advancement. This absence of an explicit politic, rather than liberating us from having to acknowledge broader constraints, constricts our ability to ask questions and hold ourselves accountable for how we approach the social implications of our work\textemdash most significantly: what social implications are acceptable or even desirable? 
}

\textcolor{blue}{
Here are people who 
are responding to the communities in which they work.
see a need and who are working from these different angles to address it in ways that we view as really valuable and impactful.
What we don't see in the academy, and what we are proposing is that we could strengthen this work, pull in the work that researchers and activists are doing on the ground, and tie together these various strands of HCI by making the politic explicit.
If we're completely comfortable coexisting alongside half of our monstrous self and not reckoning with it, how can we expect to make anything better?
There's an additional step to be made.  We have to have an explicit answer to why we want to do these things, so we have to have an explicit politic. 	
The theoretical work here highlights that HCI has a problem: that we are insufficiently cognizant of power, particularly as it relates to capital, hierarchy and axes of marginalisation. This issue is emphasised by the relative lack of application. But there is reason for hope; that there are practical applications at all show there is work to build from. In this paper\textemdash building on Linehan \& Kirman's "anarCHI" paper \cite{Linehan2014}, along with Asad's pointer to prefigurative politics \textemdash we seek to extend these critical works and political positions they stake out, weaving them into a matching coherent and explicit politic of HCI. Specifically, we wish to set out the vision of an \textit{anarchist HCI}}

\textcolor{orange}{SCRAP:
Our position is that an explicit operationalisation would be good - and further, that in line with L and K and Asad, there is a particular explicit politics that lends itself to these critical works and meaningful social awareness and change. Specifically, we advocate an explicit ANARCHIST HCI.
}

\textcolor{orange}{ SCRAP:
If we're completely comfortable coexisting alongside half of our monstrous self and not reckoning with it, how can we expect to make anything better?
There's an additional step to be made.  We have to have an explicit answer to why we want to do these things, so we have to have an explicit politic. 	
The work we have highlighted here indicates that HCI has a problem: that we are insufficiently cognizant of power, particularly as it relates to capital, hierarchy and axes of marginalisation. 
}

% \textcolor{purple}{[MD: This quote works here, but it also seems somehow more visionary than an overview of the current state of the field.]}
}

% \textcolor{purple}{
% oppression. We must illustrate, in other words, that we came ``with empty hands and a desire to unbuild walls''~\cite{Le2015}.
% }
% \textcolor{purple}{[MD - q]}

% An illustration can be seen in Sustainable HCI. Ostensibly a turn towards the social, Sustainable HCI has foregrounded issues of ecological responsibility in and through design \cite{DiSalvo2010}. But in practice, early work focused on individual actions and interventions rather than systemic challenges; the field has frequently featured that selfsame implicit neoliberalism \cite{Dourish2010}, and a failure to confront the incompatibility of sustainability with capitalism's expansionist demands \cite{Knowles2018}. 
